Electrostatic Self-energy of a Charged Particle in the Surroundings of a Topologically Charged Black Hole in the Brane

We determine the self-energy for a point charge held stationary in a topologically charged black hole spacetime arising from the Randall-Sundrum II braneworld model, showing that it has two contributions, one of geometric origin and the other of topological one.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
%that are currently in use and accepted by Romanian Journal of Physics.
% Last modified: 08/09/2013 (dd/mm/yyyy)
%
% Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}
%
% Various other operators
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\Rel}{Re}
\DeclareMathOperator{\ee}{e}
%
% Elliptic Jacobi functions - obsolete, do not use! (see below)
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}
%
% Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
% Replaceable by \tanh^{-1}
% Hyperbolic functions
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\cosech}{csch}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\cosec}{cosec}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
% Partial derivative
\providecommand{\pd}{\ensuremath{\partial}}
% To be eliminated in future versions!
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}
% Full derivative
\providecommand{\fd}{\ensuremath{\mathrm{d}}}
% Bras and Kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
% the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}
%
% Commands for multiple indexes around a central token #1
% The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
% the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
% that it reduces the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}
%
% put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}
%
% A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
% \let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%
% Jacobi elliptic functions as operators
\DeclareMathOperator{\jsn}{sn} % to replace duplicates above!
\DeclareMathOperator{\jcn}{cn}
\DeclareMathOperator{\jdn}{dn}
\DeclareMathOperator{\jns}{ns} % 1/sn(u)
\DeclareMathOperator{\jnc}{nc} % 1/cn(u)
\DeclareMathOperator{\jnd}{nd} % 1/dn(u)
\DeclareMathOperator{\jsc}{sc} % sn(u)/cn(u)
\DeclareMathOperator{\jsd}{sd} % sn(u)/dn(u)
\DeclareMathOperator{\jdc}{dc} % dn(u)/cn(u)
\DeclareMathOperator{\jds}{ds} % dn(u)/sn(u)
\DeclareMathOperator{\jcs}{cs} % cn(u)/sn(u) 
\DeclareMathOperator{\jcd}{cd} % cn(u)/dn(u)

% Pre-formatted special text chunks
\providecommand{\ie}{\textit{i.e.}}
\providecommand{\eg}{\textit{e.g.}}
\providecommand{\etal}{\textit{et al.}}



